Configuration spaces on a wedge of spheres and Hochschild-Pirashvili homology

We study the compactly supported rational cohomology of configuration spaces of points on wedges of spheres, equipped with natural actions of the symmetric group and the group $Out(F_g)$ of outer automorphisms of the free group. These representations show up in seemingly unrelated parts of mathematics, from cohomology of moduli spaces of curves to polynomial functors on free groups and Hochschild-Pirashvili cohomology. We show that these cohomology representations form a polynomial functor, and use various geometric models to compute many of its composition factors. We further compute the composition factors completely for all configurations of $n\leq 10$ particles. An application of this analysis is a new super-exponential lower bound on the symmetric group action on the weight $0$ component of $H^*_c(M_{2,n})$.

==> Decomposition_M2n.tex <==
% Not meant to be included in the paper. Only serves as a temporary notepad
2  :  0


3  :  0


4  :  s[4]


5  :  s[3, 2]


6  :  s[3, 2, 1] + s[4, 1, 1]


7  :  s[1, 1, 1, 1, 1, 1, 1] + s[2, 2, 2, 1] + s[3, 2, 1, 1] + s[3, 3, 1] + s[4, 1, 1, 1] + s[4, 2, 1] + s[4, 3] + s[5, 1, 1]


8  :  s[3, 1, 1, 1, 1, 1] + 2*s[3, 2, 1, 1, 1] + 2*s[3, 2, 2, 1] + s[3, 3, 1, 1] + s[3, 3, 2] + s[4, 1, 1, 1, 1] + 2*s[4, 2, 1, 1] + 2*s[4, 2, 2] + 2*s[4, 3, 1] + s[5, 1, 1, 1] + 2*s[5, 2, 1] + s[5, 3] + s[6, 2] + s[8]


9  :  s[1, 1, 1, 1, 1, 1, 1, 1, 1] + s[2, 2, 1, 1, 1, 1, 1] + s[2, 2, 2, 1, 1, 1] + s[2, 2, 2, 2, 1] + 3*s[3, 2, 1, 1, 1, 1] + 2*s[3, 2, 2, 1, 1] + 3*s[3, 2, 2, 2] + 4*s[3, 3, 1, 1, 1] + 4*s[3, 3, 2, 1] + s[4, 1, 1, 1, 1, 1] + 4*s[4, 2, 1, 1, 1] + 5*s[4, 2, 2, 1] + 5*s[4, 3, 1, 1] + 4*s[4, 3, 2] + 3*s[4, 4, 1] + 3*s[5, 1, 1, 1, 1] + 4*s[5, 2, 1, 1] + 5*s[5, 2, 2] + 3*s[5, 3, 1] + 2*s[5, 4] + s[6, 1, 1, 1] + 3*s[6, 2, 1] + s[6, 3] + 2*s[7, 2]


10  :  2*s[2, 2, 2, 1, 1, 1, 1] + s[2, 2, 2, 2, 1, 1] + 2*s[3, 1, 1, 1, 1, 1, 1, 1] + 3*s[3, 2, 1, 1, 1, 1, 1] + 7*s[3, 2, 2, 1, 1, 1] + 6*s[3, 2, 2, 2, 1] + 3*s[3, 3, 1, 1, 1, 1] + 10*s[3, 3, 2, 1, 1] + 4*s[3, 3, 2, 2] + 6*s[3, 3, 3, 1] + 3*s[4, 1, 1, 1, 1, 1, 1] + 8*s[4, 2, 1, 1, 1, 1] + 13*s[4, 2, 2, 1, 1] + 7*s[4, 2, 2, 2] + 11*s[4, 3, 1, 1, 1] + 16*s[4, 3, 2, 1] + 6*s[4, 3, 3] + 6*s[4, 4, 1, 1] + 6*s[4, 4, 2] + 2*s[5, 1, 1, 1, 1, 1] + 9*s[5, 2, 1, 1, 1] + 12*s[5, 2, 2, 1] + 15*s[5, 3, 1, 1] + 10*s[5, 3, 2] + 7*s[5, 4, 1] + 2*s[6, 1, 1, 1, 1] + 8*s[6, 2, 1, 1] + 4*s[6, 2, 2] + 9*s[6, 3, 1] + 2*s[6, 4] + 3*s[7, 1, 1, 1] + 4*s[7, 2, 1] + 2*s[7, 3] + 2*s[8, 1, 1]


11  :  s[1, 1, 1, 1, 1, 1, 1, 1, 1, 1, 1] + 2*s[2, 2, 1, 1, 1, 1, 1, 1, 1] + 2*s[2, 2, 2, 1, 1, 1, 1, 1] + 4*s[2, 2, 2, 2, 1, 1, 1] + 2*s[2, 2, 2, 2, 2, 1] + 6*s[3, 2, 1, 1, 1, 1, 1, 1] + 8*s[3, 2, 2, 1, 1, 1, 1] + 13*s[3, 2, 2, 2, 1, 1] + 4*s[3, 2, 2, 2, 2] + 11*s[3, 3, 1, 1, 1, 1, 1] + 18*s[3, 3, 2, 1, 1, 1] + 19*s[3, 3, 2, 2, 1] + 8*s[3, 3, 3, 1, 1] + 10*s[3, 3, 3, 2] + 2*s[4, 1, 1, 1, 1, 1, 1, 1] + 11*s[4, 2, 1, 1, 1, 1, 1] + 23*s[4, 2, 2, 1, 1, 1] + 19*s[4, 2, 2, 2, 1] + 21*s[4, 3, 1, 1, 1, 1] + 42*s[4, 3, 2, 1, 1] + 23*s[4, 3, 2, 2] + 21*s[4, 3, 3, 1] + 17*s[4, 4, 1, 1, 1] + 24*s[4, 4, 2, 1] + 7*s[4, 4, 3] + 7*s[5, 1, 1, 1, 1, 1, 1] + 17*s[5, 2, 1, 1, 1, 1] + 32*s[5, 2, 2, 1, 1] + 12*s[5, 2, 2, 2] + 25*s[5, 3, 1, 1, 1] + 42*s[5, 3, 2, 1] + 15*s[5, 3, 3] + 22*s[5, 4, 1, 1] + 16*s[5, 4, 2] + 8*s[5, 5, 1] + 5*s[6, 1, 1, 1, 1, 1] + 18*s[6, 2, 1, 1, 1] + 20*s[6, 2, 2, 1] + 23*s[6, 3, 1, 1] + 18*s[6, 3, 2] + 12*s[6, 4, 1] + 3*s[6, 5] + 2*s[7, 1, 1, 1, 1] + 12*s[7, 2, 1, 1] + 5*s[7, 2, 2] + 12*s[7, 3, 1] + 2*s[7, 4] + 2*s[8, 1, 1, 1] + 4*s[8, 2, 1] + 2*s[8, 3] + 2*s[9, 1, 1]


12  :  3*s[2, 2, 2, 1, 1, 1, 1, 1, 1] + 3*s[2, 2, 2, 2, 1, 1, 1, 1] + 5*s[2, 2, 2, 2, 2, 1, 1] + s[2, 2, 2, 2, 2, 2] + 3*s[3, 1, 1, 1, 1, 1, 1, 1, 1, 1] + 7*s[3, 2, 1, 1, 1, 1, 1, 1, 1] + 19*s[3, 2, 2, 1, 1, 1, 1, 1] + 23*s[3, 2, 2, 2, 1, 1, 1] + 20*s[3, 2, 2, 2, 2, 1] + 8*s[3, 3, 1, 1, 1, 1, 1, 1] + 34*s[3, 3, 2, 1, 1, 1, 1] + 40*s[3, 3, 2, 2, 1, 1] + 22*s[3, 3, 2, 2, 2] + 31*s[3, 3, 3, 1, 1, 1] + 34*s[3, 3, 3, 2, 1] + 4*s[3, 3, 3, 3] + 4*s[4, 1, 1, 1, 1, 1, 1, 1, 1] + 20*s[4, 2, 1, 1, 1, 1, 1, 1] + 43*s[4, 2, 2, 1, 1, 1, 1] + 52*s[4, 2, 2, 2, 1, 1] + 24*s[4, 2, 2, 2, 2] + 37*s[4, 3, 1, 1, 1, 1, 1] + 95*s[4, 3, 2, 1, 1, 1] + 93*s[4, 3, 2, 2, 1] + 69*s[4, 3, 3, 1, 1] + 48*s[4, 3, 3, 2] + 28*s[4, 4, 1, 1, 1, 1] + 73*s[4, 4, 2, 1, 1] + 40*s[4, 4, 2, 2] + 50*s[4, 4, 3, 1] + 7*s[4, 4, 4] + 5*s[5, 1, 1, 1, 1, 1, 1, 1] + 32*s[5, 2, 1, 1, 1, 1, 1] + 60*s[5, 2, 2, 1, 1, 1] + 58*s[5, 2, 2, 2, 1] + 66*s[5, 3, 1, 1, 1, 1] + 126*s[5, 3, 2, 1, 1] + 75*s[5, 3, 2, 2] + 64*s[5, 3, 3, 1] + 59*s[5, 4, 1, 1, 1] + 95*s[5, 4, 2, 1] + 35*s[5, 4, 3] + 21*s[5, 5, 1, 1] + 22*s[5, 5, 2] + 7*s[6, 1, 1, 1, 1, 1, 1] + 36*s[6, 2, 1, 1, 1, 1] + 58*s[6, 2, 2, 1, 1] + 31*s[6, 2, 2, 2] + 63*s[6, 3, 1, 1, 1] + 93*s[6, 3, 2, 1] + 25*s[6, 3, 3] + 52*s[6, 4, 1, 1] + 44*s[6, 4, 2] + 20*s[6, 5, 1] + s[6, 6] + 10*s[7, 1, 1, 1, 1, 1] + 29*s[7, 2, 1, 1, 1] + 36*s[7, 2, 2, 1] + 37*s[7, 3, 1, 1] + 33*s[7, 3, 2] + 23*s[7, 4, 1] + 6*s[7, 5] + 6*s[8, 1, 1, 1, 1] + 16*s[8, 2, 1, 1] + 11*s[8, 2, 2] + 14*s[8, 3, 1] + 5*s[8, 4] + 2*s[9, 1, 1, 1] + 6*s[9, 2, 1] + 3*s[9, 3] + 2*s[10, 2] + s[11, 1] + s[12]


13  :  2*s[1, 1, 1, 1, 1, 1, 1, 1, 1, 1, 1, 1, 1] + 3*s[2, 2, 1, 1, 1, 1, 1, 1, 1, 1, 1] + 5*s[2, 2, 2, 1, 1, 1, 1, 1, 1, 1] + 10*s[2, 2, 2, 2, 1, 1, 1, 1, 1] + 8*s[2, 2, 2, 2, 2, 1, 1, 1] + 9*s[2, 2, 2, 2, 2, 2, 1] + 9*s[3, 2, 1, 1, 1, 1, 1, 1, 1, 1] + 21*s[3, 2, 2, 1, 1, 1, 1, 1, 1] + 44*s[3, 2, 2, 2, 1, 1, 1, 1] + 39*s[3, 2, 2, 2, 2, 1, 1] + 23*s[3, 2, 2, 2, 2, 2] + 24*s[3, 3, 1, 1, 1, 1, 1, 1, 1] + 58*s[3, 3, 2, 1, 1, 1, 1, 1] + 101*s[3, 3, 2, 2, 1, 1, 1] + 77*s[3, 3, 2, 2, 2, 1] + 49*s[3, 3, 3, 1, 1, 1, 1] + 100*s[3, 3, 3, 2, 1, 1] + 42*s[3, 3, 3, 2, 2] + 44*s[3, 3, 3, 3, 1] + 5*s[4, 1, 1, 1, 1, 1, 1, 1, 1, 1] + 25*s[4, 2, 1, 1, 1, 1, 1, 1, 1] + 72*s[4, 2, 2, 1, 1, 1, 1, 1] + 106*s[4, 2, 2, 2, 1, 1, 1] + 86*s[4, 2, 2, 2, 2, 1] + 64*s[4, 3, 1, 1, 1, 1, 1, 1] + 190*s[4, 3, 2, 1, 1, 1, 1] + 261*s[4, 3, 2, 2, 1, 1] + 130*s[4, 3, 2, 2, 2] + 175*s[4, 3, 3, 1, 1, 1] + 221*s[4, 3, 3, 2, 1] + 52*s[4, 3, 3, 3] + 74*s[4, 4, 1, 1, 1, 1, 1] + 184*s[4, 4, 2, 1, 1, 1] + 198*s[4, 4, 2, 2, 1] + 165*s[4, 4, 3, 1, 1] + 129*s[4, 4, 3, 2] + 53*s[4, 4, 4, 1] + 14*s[5, 1, 1, 1, 1, 1, 1, 1, 1] + 51*s[5, 2, 1, 1, 1, 1, 1, 1] + 136*s[5, 2, 2, 1, 1, 1, 1] + 153*s[5, 2, 2, 2, 1, 1] + 82*s[5, 2, 2, 2, 2] + 110*s[5, 3, 1, 1, 1, 1, 1] + 318*s[5, 3, 2, 1, 1, 1] + 315*s[5, 3, 2, 2, 1] + 256*s[5, 3, 3, 1, 1] + 163*s[5, 3, 3, 2] + 142*s[5, 4, 1, 1, 1, 1] + 316*s[5, 4, 2, 1, 1] + 196*s[5, 4, 2, 2] + 220*s[5, 4, 3, 1] + 43*s[5, 4, 4] + 83*s[5, 5, 1, 1, 1] + 130*s[5, 5, 2, 1] + 43*s[5, 5, 3] + 14*s[6, 1, 1, 1, 1, 1, 1, 1] + 72*s[6, 2, 1, 1, 1, 1, 1] + 146*s[6, 2, 2, 1, 1, 1] + 137*s[6, 2, 2, 2, 1] + 146*s[6, 3, 1, 1, 1, 1] + 311*s[6, 3, 2, 1, 1] + 179*s[6, 3, 2, 2] + 171*s[6, 3, 3, 1] + 152*s[6, 4, 1, 1, 1] + 256*s[6, 4, 2, 1] + 98*s[6, 4, 3] + 85*s[6, 5, 1, 1] + 77*s[6, 5, 2] + 22*s[6, 6, 1] + 12*s[7, 1, 1, 1, 1, 1, 1] + 69*s[7, 2, 1, 1, 1, 1] + 104*s[7, 2, 2, 1, 1] + 68*s[7, 2, 2, 2] + 128*s[7, 3, 1, 1, 1] + 178*s[7, 3, 2, 1] + 46*s[7, 3, 3] + 102*s[7, 4, 1, 1] + 95*s[7, 4, 2] + 39*s[7, 5, 1] + 9*s[7, 6] + 12*s[8, 1, 1, 1, 1, 1] + 45*s[8, 2, 1, 1, 1] + 56*s[8, 2, 2, 1] + 64*s[8, 3, 1, 1] + 52*s[8, 3, 2] + 40*s[8, 4, 1] + 8*s[8, 5] + 11*s[9, 1, 1, 1, 1] + 20*s[9, 2, 1, 1] + 19*s[9, 2, 2] + 18*s[9, 3, 1] + 8*s[9, 4] + 4*s[10, 1, 1, 1] + 7*s[10, 2, 1] + 4*s[10, 3] + 2*s[11, 2] + s[13]


14  :  5*s[2, 2, 2, 1, 1, 1, 1, 1, 1, 1, 1] + 8*s[2, 2, 2, 2, 1, 1, 1, 1, 1, 1] + 16*s[2, 2, 2, 2, 2, 1, 1, 1, 1] + 12*s[2, 2, 2, 2, 2, 2, 1, 1] + 8*s[2, 2, 2, 2, 2, 2, 2] + 5*s[3, 1, 1, 1, 1, 1, 1, 1, 1, 1, 1, 1] + 12*s[3, 2, 1, 1, 1, 1, 1, 1, 1, 1, 1] + 40*s[3, 2, 2, 1, 1, 1, 1, 1, 1, 1] + 70*s[3, 2, 2, 2, 1, 1, 1, 1, 1] + 94*s[3, 2, 2, 2, 2, 1, 1, 1] + 65*s[3, 2, 2, 2, 2, 2, 1] + 18*s[3, 3, 1, 1, 1, 1, 1, 1, 1, 1] + 95*s[3, 3, 2, 1, 1, 1, 1, 1, 1] + 172*s[3, 3, 2, 2, 1, 1, 1, 1] + 205*s[3, 3, 2, 2, 2, 1, 1] + 83*s[3, 3, 2, 2, 2, 2] + 118*s[3, 3, 3, 1, 1, 1, 1, 1] + 231*s[3, 3, 3, 2, 1, 1, 1] + 216*s[3, 3, 3, 2, 2, 1] + 114*s[3, 3, 3, 3, 1, 1] + 88*s[3, 3, 3, 3, 2] + 6*s[4, 1, 1, 1, 1, 1, 1, 1, 1, 1, 1] + 42*s[4, 2, 1, 1, 1, 1, 1, 1, 1, 1] + 118*s[4, 2, 2, 1, 1, 1, 1, 1, 1] + 214*s[4, 2, 2, 2, 1, 1, 1, 1] + 224*s[4, 2, 2, 2, 2, 1, 1] + 103*s[4, 2, 2, 2, 2, 2] + 100*s[4, 3, 1, 1, 1, 1, 1, 1, 1] + 360*s[4, 3, 2, 1, 1, 1, 1, 1] + 610*s[4, 3, 2, 2, 1, 1, 1] + 515*s[4, 3, 2, 2, 2, 1] + 396*s[4, 3, 3, 1, 1, 1, 1] + 705*s[4, 3, 3, 2, 1, 1] + 373*s[4, 3, 3, 2, 2] + 287*s[4, 3, 3, 3, 1] + 107*s[4, 4, 1, 1, 1, 1, 1, 1] + 410*s[4, 4, 2, 1, 1, 1, 1] + 576*s[4, 4, 2, 2, 1, 1] + 302*s[4, 4, 2, 2, 2] + 505*s[4, 4, 3, 1, 1, 1] + 662*s[4, 4, 3, 2, 1] + 154*s[4, 4, 3, 3] + 206*s[4, 4, 4, 1, 1] + 168*s[4, 4, 4, 2] + 10*s[5, 1, 1, 1, 1, 1, 1, 1, 1, 1] + 84*s[5, 2, 1, 1, 1, 1, 1, 1, 1] + 225*s[5, 2, 2, 1, 1, 1, 1, 1] + 366*s[5, 2, 2, 2, 1, 1, 1] + 292*s[5, 2, 2, 2, 2, 1] + 231*s[5, 3, 1, 1, 1, 1, 1, 1] + 700*s[5, 3, 2, 1, 1, 1, 1] + 994*s[5, 3, 2, 2, 1, 1] + 478*s[5, 3, 2, 2, 2] + 660*s[5, 3, 3, 1, 1, 1] + 884*s[5, 3, 3, 2, 1] + 215*s[5, 3, 3, 3] + 300*s[5, 4, 1, 1, 1, 1, 1] + 896*s[5, 4, 2, 1, 1, 1] + 947*s[5, 4, 2, 2, 1] + 884*s[5, 4, 3, 1, 1] + 655*s[5, 4, 3, 2] + 281*s[5, 4, 4, 1] + 185*s[5, 5, 1, 1, 1, 1] + 487*s[5, 5, 2, 1, 1] + 280*s[5, 5, 2, 2] + 380*s[5, 5, 3, 1] + 80*s[5, 5, 4] + 21*s[6, 1, 1, 1, 1, 1, 1, 1, 1] + 125*s[6, 2, 1, 1, 1, 1, 1, 1] + 314*s[6, 2, 2, 1, 1, 1, 1] + 403*s[6, 2, 2, 2, 1, 1] + 195*s[6, 2, 2, 2, 2] + 314*s[6, 3, 1, 1, 1, 1, 1] + 850*s[6, 3, 2, 1, 1, 1] + 875*s[6, 3, 2, 2, 1] + 661*s[6, 3, 3, 1, 1] + 479*s[6, 3, 3, 2] + 416*s[6, 4, 1, 1, 1, 1] + 964*s[6, 4, 2, 1, 1] + 582*s[6, 4, 2, 2] + 679*s[6, 4, 3, 1] + 122*s[6, 4, 4] + 292*s[6, 5, 1, 1, 1] + 501*s[6, 5, 2, 1] + 206*s[6, 5, 3] + 90*s[6, 6, 1, 1] + 91*s[6, 6, 2] + 31*s[7, 1, 1, 1, 1, 1, 1, 1] + 141*s[7, 2, 1, 1, 1, 1, 1] + 308*s[7, 2, 2, 1, 1, 1] + 283*s[7, 2, 2, 2, 1] + 297*s[7, 3, 1, 1, 1, 1] + 668*s[7, 3, 2, 1, 1] + 377*s[7, 3, 2, 2] + 380*s[7, 3, 3, 1] + 348*s[7, 4, 1, 1, 1] + 576*s[7, 4, 2, 1] + 218*s[7, 4, 3] + 222*s[7, 5, 1, 1] + 188*s[7, 5, 2] + 63*s[7, 6, 1] + 4*s[7, 7] + 27*s[8, 1, 1, 1, 1, 1, 1] + 118*s[8, 2, 1, 1, 1, 1] + 200*s[8, 2, 2, 1, 1] + 106*s[8, 2, 2, 2] + 209*s[8, 3, 1, 1, 1] + 323*s[8, 3, 2, 1] + 98*s[8, 3, 3] + 187*s[8, 4, 1, 1] + 165*s[8, 4, 2] + 84*s[8, 5, 1] + 15*s[8, 6] + 16*s[9, 1, 1, 1, 1, 1] + 71*s[9, 2, 1, 1, 1] + 82*s[9, 2, 2, 1] + 104*s[9, 3, 1, 1] + 78*s[9, 3, 2] + 61*s[9, 4, 1] + 12*s[9, 5] + 9*s[10, 1, 1, 1, 1] + 30*s[10, 2, 1, 1] + 19*s[10, 2, 2] + 30*s[10, 3, 1] + 9*s[10, 4] + 6*s[11, 1, 1, 1] + 9*s[11, 2, 1] + 3*s[11, 3] + 4*s[12, 1, 1] + s[12, 2]


15  :  2*s[1, 1, 1, 1, 1, 1, 1, 1, 1, 1, 1, 1, 1, 1, 1] + 5*s[2, 2, 1, 1, 1, 1, 1, 1, 1, 1, 1, 1, 1] + 7*s[2, 2, 2, 1, 1, 1, 1, 1, 1, 1, 1, 1] + 20*s[2, 2, 2, 2, 1, 1, 1, 1, 1, 1, 1] + 25*s[2, 2, 2, 2, 2, 1, 1, 1, 1, 1] + 33*s[2, 2, 2, 2, 2, 2, 1, 1, 1] + 20*s[2, 2, 2, 2, 2, 2, 2, 1] + 16*s[3, 2, 1, 1, 1, 1, 1, 1, 1, 1, 1, 1] + 44*s[3, 2, 2, 1, 1, 1, 1, 1, 1, 1, 1] + 113*s[3, 2, 2, 2, 1, 1, 1, 1, 1, 1] + 159*s[3, 2, 2, 2, 2, 1, 1, 1, 1] + 167*s[3, 2, 2, 2, 2, 2, 1, 1] + 59*s[3, 2, 2, 2, 2, 2, 2] + 46*s[3, 3, 1, 1, 1, 1, 1, 1, 1, 1, 1] + 147*s[3, 3, 2, 1, 1, 1, 1, 1, 1, 1] + 344*s[3, 3, 2, 2, 1, 1, 1, 1, 1] + 446*s[3, 3, 2, 2, 2, 1, 1, 1] + 347*s[3, 3, 2, 2, 2, 2, 1] + 168*s[3, 3, 3, 1, 1, 1, 1, 1, 1] + 495*s[3, 3, 3, 2, 1, 1, 1, 1] + 582*s[3, 3, 3, 2, 2, 1, 1] + 297*s[3, 3, 3, 2, 2, 2] + 358*s[3, 3, 3, 3, 1, 1, 1] + 394*s[3, 3, 3, 3, 2, 1] + 62*s[3, 3, 3, 3, 3] + 7*s[4, 1, 1, 1, 1, 1, 1, 1, 1, 1, 1, 1] + 49*s[4, 2, 1, 1, 1, 1, 1, 1, 1, 1, 1] + 180*s[4, 2, 2, 1, 1, 1, 1, 1, 1, 1] + 363*s[4, 2, 2, 2, 1, 1, 1, 1, 1] + 492*s[4, 2, 2, 2, 2, 1, 1, 1] + 361*s[4, 2, 2, 2, 2, 2, 1] + 155*s[4, 3, 1, 1, 1, 1, 1, 1, 1, 1] + 630*s[4, 3, 2, 1, 1, 1, 1, 1, 1] + 1277*s[4, 3, 2, 2, 1, 1, 1, 1] + 1456*s[4, 3, 2, 2, 2, 1, 1] + 661*s[4, 3, 2, 2, 2, 2] + 805*s[4, 3, 3, 1, 1, 1, 1, 1] + 1810*s[4, 3, 3, 2, 1, 1, 1] + 1685*s[4, 3, 3, 2, 2, 1] + 1044*s[4, 3, 3, 3, 1, 1] + 696*s[4, 3, 3, 3, 2] + 222*s[4, 4, 1, 1, 1, 1, 1, 1, 1] + 830*s[4, 4, 2, 1, 1, 1, 1, 1] + 1535*s[4, 4, 2, 2, 1, 1, 1] + 1309*s[4, 4, 2, 2, 2, 1] + 1184*s[4, 4, 3, 1, 1, 1, 1] + 2293*s[4, 4, 3, 2, 1, 1] + 1221*s[4, 4, 3, 2, 2] + 1061*s[4, 4, 3, 3, 1] + 650*s[4, 4, 4, 1, 1, 1] + 955*s[4, 4, 4, 2, 1] + 302*s[4, 4, 4, 3] + 26*s[5, 1, 1, 1, 1, 1, 1, 1, 1, 1, 1] + 126*s[5, 2, 1, 1, 1, 1, 1, 1, 1, 1] + 423*s[5, 2, 2, 1, 1, 1, 1, 1, 1] + 748*s[5, 2, 2, 2, 1, 1, 1, 1] + 853*s[5, 2, 2, 2, 2, 1, 1] + 352*s[5, 2, 2, 2, 2, 2] + 356*s[5, 3, 1, 1, 1, 1, 1, 1, 1] + 1414*s[5, 3, 2, 1, 1, 1, 1, 1] + 2459*s[5, 3, 2, 2, 1, 1, 1] + 2128*s[5, 3, 2, 2, 2, 1] + 1701*s[5, 3, 3, 1, 1, 1, 1] + 3010*s[5, 3, 3, 2, 1, 1] + 1667*s[5, 3, 3, 2, 2] + 1254*s[5, 3, 3, 3, 1] + 599*s[5, 4, 1, 1, 1, 1, 1, 1] + 2131*s[5, 4, 2, 1, 1, 1, 1] + 3193*s[5, 4, 2, 2, 1, 1] + 1591*s[5, 4, 2, 2, 2] + 2743*s[5, 4, 3, 1, 1, 1] + 3751*s[5, 4, 3, 2, 1] + 960*s[5, 4, 3, 3] + 1309*s[5, 4, 4, 1, 1] + 1007*s[5, 4, 4, 2] + 494*s[5, 5, 1, 1, 1, 1, 1] + 1464*s[5, 5, 2, 1, 1, 1] + 1628*s[5, 5, 2, 2, 1] + 1572*s[5, 5, 3, 1, 1] + 1244*s[5, 5, 3, 2] + 684*s[5, 5, 4, 1] + 87*s[5, 5, 5] + 33*s[6, 1, 1, 1, 1, 1, 1, 1, 1, 1] + 223*s[6, 2, 1, 1, 1, 1, 1, 1, 1] + 633*s[6, 2, 2, 1, 1, 1, 1, 1] + 1022*s[6, 2, 2, 2, 1, 1, 1] + 840*s[6, 2, 2, 2, 2, 1] + 612*s[6, 3, 1, 1, 1, 1, 1, 1] + 2032*s[6, 3, 2, 1, 1, 1, 1] + 2898*s[6, 3, 2, 2, 1, 1] + 1445*s[6, 3, 2, 2, 2] + 2040*s[6, 3, 3, 1, 1, 1] + 2703*s[6, 3, 3, 2, 1] + 633*s[6, 3, 3, 3] + 934*s[6, 4, 1, 1, 1, 1, 1] + 2896*s[6, 4, 2, 1, 1, 1] + 3111*s[6, 4, 2, 2, 1] + 2986*s[6, 4, 3, 1, 1] + 2217*s[6, 4, 3, 2] + 1013*s[6, 4, 4, 1] + 838*s[6, 5, 1, 1, 1, 1] + 2082*s[6, 5, 2, 1, 1] + 1269*s[6, 5, 2, 2] + 1631*s[6, 5, 3, 1] + 380*s[6, 5, 4] + 377*s[6, 6, 1, 1, 1] + 637*s[6, 6, 2, 1] + 256*s[6, 6, 3] + 37*s[7, 1, 1, 1, 1, 1, 1, 1, 1] + 279*s[7, 2, 1, 1, 1, 1, 1, 1] + 684*s[7, 2, 2, 1, 1, 1, 1] + 936*s[7, 2, 2, 2, 1, 1] + 420*s[7, 2, 2, 2, 2] + 731*s[7, 3, 1, 1, 1, 1, 1] + 1975*s[7, 3, 2, 1, 1, 1] + 2067*s[7, 3, 2, 2, 1] + 1537*s[7, 3, 3, 1, 1] + 1171*s[7, 3, 3, 2] + 980*s[7, 4, 1, 1, 1, 1] + 2393*s[7, 4, 2, 1, 1] + 1407*s[7, 4, 2, 2] + 1720*s[7, 4, 3, 1] + 294*s[7, 4, 4] + 770*s[7, 5, 1, 1, 1] + 1376*s[7, 5, 2, 1] + 590*s[7, 5, 3] + 349*s[7, 6, 1, 1] + 311*s[7, 6, 2] + 70*s[7, 7, 1] + 49*s[8, 1, 1, 1, 1, 1, 1, 1] + 261*s[8, 2, 1, 1, 1, 1, 1] + 570*s[8, 2, 2, 1, 1, 1] + 544*s[8, 2, 2, 2, 1] + 591*s[8, 3, 1, 1, 1, 1] + 1297*s[8, 3, 2, 1, 1] + 755*s[8, 3, 2, 2] + 732*s[8, 3, 3, 1] + 703*s[8, 4, 1, 1, 1] + 1163*s[8, 4, 2, 1] + 441*s[8, 4, 3] + 450*s[8, 5, 1, 1] + 406*s[8, 5, 2] + 144*s[8, 6, 1] + 19*s[8, 7] + 49*s[9, 1, 1, 1, 1, 1, 1] + 189*s[9, 2, 1, 1, 1, 1] + 345*s[9, 2, 2, 1, 1] + 162*s[9, 2, 2, 2] + 338*s[9, 3, 1, 1, 1] + 545*s[9, 3, 2, 1] + 179*s[9, 3, 3] + 330*s[9, 4, 1, 1] + 272*s[9, 4, 2] + 154*s[9, 5, 1] + 23*s[9, 6] + 27*s[10, 1, 1, 1, 1, 1] + 105*s[10, 2, 1, 1, 1] + 126*s[10, 2, 2, 1] + 147*s[10, 3, 1, 1] + 120*s[10, 3, 2] + 90*s[10, 4, 1] + 21*s[10, 5] + 10*s[11, 1, 1, 1, 1] + 44*s[11, 2, 1, 1] + 19*s[11, 2, 2] + 44*s[11, 3, 1] + 10*s[11, 4] + 5*s[12, 1, 1, 1] + 11*s[12, 2, 1] + 5*s[12, 3] + 4*s[13, 1, 1]


16  :  10*s[2, 2, 2, 1, 1, 1, 1, 1, 1, 1, 1, 1, 1] + 16*s[2, 2, 2, 2, 1, 1, 1, 1, 1, 1, 1, 1] + 39*s[2, 2, 2, 2, 2, 1, 1, 1, 1, 1, 1] + 47*s[2, 2, 2, 2, 2, 2, 1, 1, 1, 1] + 49*s[2, 2, 2, 2, 2, 2, 2, 1, 1] + 12*s[2, 2, 2, 2, 2, 2, 2, 2] + 7*s[3, 1, 1, 1, 1, 1, 1, 1, 1, 1, 1, 1, 1, 1] + 18*s[3, 2, 1, 1, 1, 1, 1, 1, 1, 1, 1, 1, 1] + 76*s[3, 2, 2, 1, 1, 1, 1, 1, 1, 1, 1, 1] + 167*s[3, 2, 2, 2, 1, 1, 1, 1, 1, 1, 1] + 295*s[3, 2, 2, 2, 2, 1, 1, 1, 1, 1] + 339*s[3, 2, 2, 2, 2, 2, 1, 1, 1] + 241*s[3, 2, 2, 2, 2, 2, 2, 1] + 35*s[3, 3, 1, 1, 1, 1, 1, 1, 1, 1, 1, 1] + 220*s[3, 3, 2, 1, 1, 1, 1, 1, 1, 1, 1] + 531*s[3, 3, 2, 2, 1, 1, 1, 1, 1, 1] + 895*s[3, 3, 2, 2, 2, 1, 1, 1, 1] + 872*s[3, 3, 2, 2, 2, 2, 1, 1] + 399*s[3, 3, 2, 2, 2, 2, 2] + 345*s[3, 3, 3, 1, 1, 1, 1, 1, 1, 1] + 949*s[3, 3, 3, 2, 1, 1, 1, 1, 1] + 1476*s[3, 3, 3, 2, 2, 1, 1, 1] + 1160*s[3, 3, 3, 2, 2, 2, 1] + 740*s[3, 3, 3, 3, 1, 1, 1, 1] + 1265*s[3, 3, 3, 3, 2, 1, 1] + 610*s[3, 3, 3, 3, 2, 2] + 463*s[3, 3, 3, 3, 3, 1] + 11*s[4, 1, 1, 1, 1, 1, 1, 1, 1, 1, 1, 1, 1] + 78*s[4, 2, 1, 1, 1, 1, 1, 1, 1, 1, 1, 1] + 270*s[4, 2, 2, 1, 1, 1, 1, 1, 1, 1, 1] + 641*s[4, 2, 2, 2, 1, 1, 1, 1, 1, 1] + 974*s[4, 2, 2, 2, 2, 1, 1, 1, 1] + 978*s[4, 2, 2, 2, 2, 2, 1, 1] + 404*s[4, 2, 2, 2, 2, 2, 2] + 229*s[4, 3, 1, 1, 1, 1, 1, 1, 1, 1, 1] + 1043*s[4, 3, 2, 1, 1, 1, 1, 1, 1, 1] + 2454*s[4, 3, 2, 2, 1, 1, 1, 1, 1] + 3466*s[4, 3, 2, 2, 2, 1, 1, 1] + 2654*s[4, 3, 2, 2, 2, 2, 1] + 1533*s[4, 3, 3, 1, 1, 1, 1, 1, 1] + 4140*s[4, 3, 3, 2, 1, 1, 1, 1] + 5237*s[4, 3, 3, 2, 2, 1, 1] + 2485*s[4, 3, 3, 2, 2, 2] + 3007*s[4, 3, 3, 3, 1, 1, 1] + 3590*s[4, 3, 3, 3, 2, 1] + 732*s[4, 3, 3, 3, 3] + 318*s[4, 4, 1, 1, 1, 1, 1, 1, 1, 1] + 1566*s[4, 4, 2, 1, 1, 1, 1, 1, 1] + 3354*s[4, 4, 2, 2, 1, 1, 1, 1] + 4038*s[4, 4, 2, 2, 2, 1, 1] + 1815*s[4, 4, 2, 2, 2, 2] + 2714*s[4, 4, 3, 1, 1, 1, 1, 1] + 6407*s[4, 4, 3, 2, 1, 1, 1] + 6154*s[4, 4, 3, 2, 2, 1] + 4049*s[4, 4, 3, 3, 1, 1] + 2820*s[4, 4, 3, 3, 2] + 1758*s[4, 4, 4, 1, 1, 1, 1] + 3687*s[4, 4, 4, 2, 1, 1] + 2047*s[4, 4, 4, 2, 2] + 2161*s[4, 4, 4, 3, 1] + 272*s[4, 4, 4, 4] + 19*s[5, 1, 1, 1, 1, 1, 1, 1, 1, 1, 1, 1] + 188*s[5, 2, 1, 1, 1, 1, 1, 1, 1, 1, 1] + 656*s[5, 2, 2, 1, 1, 1, 1, 1, 1, 1] + 1446*s[5, 2, 2, 2, 1, 1, 1, 1, 1] + 1936*s[5, 2, 2, 2, 2, 1, 1, 1] + 1481*s[5, 2, 2, 2, 2, 2, 1] + 645*s[5, 3, 1, 1, 1, 1, 1, 1, 1, 1] + 2654*s[5, 3, 2, 1, 1, 1, 1, 1, 1] + 5615*s[5, 3, 2, 2, 1, 1, 1, 1] + 6473*s[5, 3, 2, 2, 2, 1, 1] + 3004*s[5, 3, 2, 2, 2, 2] + 3586*s[5, 3, 3, 1, 1, 1, 1, 1] + 8439*s[5, 3, 3, 2, 1, 1, 1] + 7920*s[5, 3, 3, 2, 2, 1] + 5088*s[5, 3, 3, 3, 1, 1] + 3355*s[5, 3, 3, 3, 2] + 1105*s[5, 4, 1, 1, 1, 1, 1, 1, 1] + 4696*s[5, 4, 2, 1, 1, 1, 1, 1] + 8748*s[5, 4, 2, 2, 1, 1, 1] + 7738*s[5, 4, 2, 2, 2, 1] + 7276*s[5, 4, 3, 1, 1, 1, 1] + 14062*s[5, 4, 3, 2, 1, 1] + 7724*s[5, 4, 3, 2, 2] + 6587*s[5, 4, 3, 3, 1] + 4353*s[5, 4, 4, 1, 1, 1] + 6581*s[5, 4, 4, 2, 1] + 2157*s[5, 4, 4, 3] + 951*s[5, 5, 1, 1, 1, 1, 1, 1] + 3835*s[5, 5, 2, 1, 1, 1, 1] + 5795*s[5, 5, 2, 2, 1, 1] + 3045*s[5, 5, 2, 2, 2] + 5518*s[5, 5, 3, 1, 1, 1] + 7679*s[5, 5, 3, 2, 1] + 1980*s[5, 5, 3, 3] + 3341*s[5, 5, 4, 1, 1] + 2769*s[5, 5, 4, 2] + 697*s[5, 5, 5, 1] + 47*s[6, 1, 1, 1, 1, 1, 1, 1, 1, 1, 1] + 347*s[6, 2, 1, 1, 1, 1, 1, 1, 1, 1] + 1175*s[6, 2, 2, 1, 1, 1, 1, 1, 1] + 2243*s[6, 2, 2, 2, 1, 1, 1, 1] + 2519*s[6, 2, 2, 2, 2, 1, 1] + 1127*s[6, 2, 2, 2, 2, 2] + 1137*s[6, 3, 1, 1, 1, 1, 1, 1, 1] + 4400*s[6, 3, 2, 1, 1, 1, 1, 1] + 7913*s[6, 3, 2, 2, 1, 1, 1] + 6859*s[6, 3, 2, 2, 2, 1] + 5364*s[6, 3, 3, 1, 1, 1, 1] + 9990*s[6, 3, 3, 2, 1, 1] + 5406*s[6, 3, 3, 2, 2] + 4331*s[6, 3, 3, 3, 1] + 2047*s[6, 4, 1, 1, 1, 1, 1, 1] + 7522*s[6, 4, 2, 1, 1, 1, 1] + 11378*s[6, 4, 2, 2, 1, 1] + 5775*s[6, 4, 2, 2, 2] + 9947*s[6, 4, 3, 1, 1, 1] + 13828*s[6, 4, 3, 2, 1] + 3590*s[6, 4, 3, 3] + 4923*s[6, 4, 4, 1, 1] + 3973*s[6, 4, 4, 2] + 2102*s[6, 5, 1, 1, 1, 1, 1] + 6814*s[6, 5, 2, 1, 1, 1] + 7559*s[6, 5, 2, 2, 1] + 7765*s[6, 5, 3, 1, 1] + 5939*s[6, 5, 3, 2] + 3460*s[6, 5, 4, 1] + 424*s[6, 5, 5] + 1086*s[6, 6, 1, 1, 1, 1] + 2885*s[6, 6, 2, 1, 1] + 1746*s[6, 6, 2, 2] + 2398*s[6, 6, 3, 1] + 599*s[6, 6, 4] + 86*s[7, 1, 1, 1, 1, 1, 1, 1, 1, 1] + 504*s[7, 2, 1, 1, 1, 1, 1, 1, 1] + 1535*s[7, 2, 2, 1, 1, 1, 1, 1] + 2480*s[7, 2, 2, 2, 1, 1, 1] + 2080*s[7, 2, 2, 2, 2, 1] + 1468*s[7, 3, 1, 1, 1, 1, 1, 1] + 5076*s[7, 3, 2, 1, 1, 1, 1] + 7313*s[7, 3, 2, 2, 1, 1] + 3720*s[7, 3, 2, 2, 2] + 5289*s[7, 3, 3, 1, 1, 1] + 6994*s[7, 3, 3, 2, 1] + 1640*s[7, 3, 3, 3] + 2481*s[7, 4, 1, 1, 1, 1, 1] + 7685*s[7, 4, 2, 1, 1, 1] + 8399*s[7, 4, 2, 2, 1] + 8075*s[7, 4, 3, 1, 1] + 6085*s[7, 4, 3, 2] + 2869*s[7, 4, 4, 1] + 2483*s[7, 5, 1, 1, 1, 1] + 6176*s[7, 5, 2, 1, 1] + 3848*s[7, 5, 2, 2] + 4909*s[7, 5, 3, 1] + 1185*s[7, 5, 4] + 1401*s[7, 6, 1, 1, 1] + 2493*s[7, 6, 2, 1] + 1082*s[7, 6, 3] + 362*s[7, 7, 1, 1] + 366*s[7, 7, 2] + 91*s[8, 1, 1, 1, 1, 1, 1, 1, 1] + 557*s[8, 2, 1, 1, 1, 1, 1, 1] + 1452*s[8, 2, 2, 1, 1, 1, 1] + 1916*s[8, 2, 2, 2, 1, 1] + 926*s[8, 2, 2, 2, 2] + 1456*s[8, 3, 1, 1, 1, 1, 1] + 4147*s[8, 3, 2, 1, 1, 1] + 4346*s[8, 3, 2, 2, 1] + 3383*s[8, 3, 3, 1, 1] + 2461*s[8, 3, 3, 2] + 2112*s[8, 4, 1, 1, 1, 1] + 5163*s[8, 4, 2, 1, 1] + 3113*s[8, 4, 2, 2] + 3795*s[8, 4, 3, 1] + 709*s[8, 4, 4] + 1810*s[8, 5, 1, 1, 1] + 3172*s[8, 5, 2, 1] + 1320*s[8, 5, 3] + 891*s[8, 6, 1, 1] + 808*s[8, 6, 2] + 214*s[8, 7, 1] + 12*s[8, 8] + 77*s[9, 1, 1, 1, 1, 1, 1, 1] + 466*s[9, 2, 1, 1, 1, 1, 1] + 1007*s[9, 2, 2, 1, 1, 1] + 983*s[9, 2, 2, 2, 1] + 1083*s[9, 3, 1, 1, 1, 1] + 2352*s[9, 3, 2, 1, 1] + 1398*s[9, 3, 2, 2] + 1326*s[9, 3, 3, 1] + 1281*s[9, 4, 1, 1, 1] + 2167*s[9, 4, 2, 1] + 832*s[9, 4, 3] + 839*s[9, 5, 1, 1] + 791*s[9, 5, 2] + 298*s[9, 6, 1] + 46*s[9, 7] + 64*s[10, 1, 1, 1, 1, 1, 1] + 300*s[10, 2, 1, 1, 1, 1] + 517*s[10, 2, 2, 1, 1] + 285*s[10, 2, 2, 2] + 571*s[10, 3, 1, 1, 1] + 872*s[10, 3, 2, 1] + 263*s[10, 3, 3] + 531*s[10, 4, 1, 1] + 463*s[10, 4, 2] + 240*s[10, 5, 1] + 44*s[10, 6] + 44*s[11, 1, 1, 1, 1, 1] + 148*s[11, 2, 1, 1, 1] + 186*s[11, 2, 2, 1] + 204*s[11, 3, 1, 1] + 178*s[11, 3, 2] + 134*s[11, 4, 1] + 35*s[11, 5] + 20*s[12, 1, 1, 1, 1] + 54*s[12, 2, 1, 1] + 37*s[12, 2, 2] + 51*s[12, 3, 1] + 16*s[12, 4] + 6*s[13, 1, 1, 1] + 13*s[13, 2, 1] + 9*s[13, 3] + s[14, 1, 1] + 4*s[14, 2] + s[15, 1] + 2*s[16]


17 : s[17] + 4*s[15,2] + 8*s[14,3] + 17*s[14,2,1] + 8*s[14,1^3] + 26*s[13,4] + 61*s[13,3,1] + 58*s[13,2^2] + 65*s[13,2,1^2] + 31*s[13,1^4] + 46*s[12,5] + 193*s[12,4,1] + 246*s[12,3,2] + 300*s[12,3,1^2] + 254*s[12,2^2,1] + 207*s[12,2,1^3] + 54*s[12,1^5] + 76*s[11,6] + 371*s[11,5,1] + 748*s[11,4,2] + 807*s[11,4,1^2] + 381*s[11,3^2] + 1356*s[11,3,2,1] + 897*s[11,3,1^3] + 462*s[11,2^3] + 769*s[11,2^2,1^2] + 470*s[11,2,1^4] + 85*s[11,1^6] + 80*s[10,7] + 555*s[10,6,1] + 1397*s[10,5,2] + 1526*s[10,5,1^2] + 1470*s[10,4,3] + 3781*s[10,4,2,1] + 2218*s[10,4,1^3] + 2335*s[10,3^2,1] + 2386*s[10,3,2^2] + 4060*s[10,3,2,1^2] + 1815*s[10,3,1^4] + 1684*s[10,2^3,1] + 1737*s[10,2^2,1^3] + 790*s[10,2,1^5] + 141*s[10,1^7] + 58*s[9,8] + 504*s[9,7,1] + 1798*s[9,6,2] + 1896*s[9,6,1^2] + 2711*s[9,5,3] + 6544*s[9,5,2,1] + 3756*s[9,5,1^3] + 1500*s[9,4^2] + 7623*s[9,4,3,1] + 6323*s[9,4,2^2] + 10253*s[9,4,2,1^2] + 4221*s[9,4,1^4] + 4816*s[9,3^2,2] + 6749*s[9,3^2,1^2] + 8498*s[9,3,2^2,1] + 8077*s[9,3,2,1^3] + 2766*s[9,3,1^5] + 1859*s[9,2^4] + 3649*s[9,2^3,1^2] + 2810*s[9,2^2,1^4] + 1033*s[9,2,1^6] + 183*s[9,1^8] + 229*s[8^2,1] + 1298*s[8,7,2] + 1382*s[8,7,1^2] + 3043*s[8,6,3] + 6907*s[8,6,2,1] + 3806*s[8,6,1^3] + 3019*s[8,5,4] + 12424*s[8,5,3,1] + 9496*s[8,5,2^2] + 15346*s[8,5,2,1^2] + 5998*s[8,5,1^4] + 6899*s[8,4^2,1] + 14551*s[8,4,3,2] + 19154*s[8,4,3,1^2] + 19814*s[8,4,2^2,1] + 18006*s[8,4,2,1^3] + 5734*s[8,4,1^5] + 3882*s[8,3^3] + 16162*s[8,3^2,2,1] + 12003*s[8,3^2,1^3] + 8448*s[8,3,2^3] + 16715*s[8,3,2^2,1^2] + 11421*s[8,3,2,1^4] + 3307*s[8,3,1^6] + 4621*s[8,2^4,1] + 5480*s[8,2^3,1^3] + 3305*s[8,2^2,1^5] + 1072*s[8,2,1^7] + 153*s[8,1^9] + 1302*s[7^2,3] + 3034*s[7^2,2,1] + 1719*s[7^2,1^3] + 2717*s[7,6,4] + 10220*s[7,6,3,1] + 7631*s[7,6,2^2] + 12150*s[7,6,2,1^2] + 4679*s[7,6,1^4] + 1448*s[7,5^2] + 11683*s[7,5,4,1] + 19466*s[7,5,3,2] + 25499*s[7,5,3,1^2] + 24355*s[7,5,2^2,1] + 21784*s[7,5,2,1^3] + 6538*s[7,5,1^5] + 12248*s[7,4^2,2] + 14787*s[7,4^2,1^2] + 10617*s[7,4,3^2] + 40842*s[7,4,3,2,1] + 29188*s[7,4,3,1^3] + 16937*s[7,4,2^3] + 32702*s[7,4,2^2,1^2] + 21513*s[7,4,2,1^4] + 5631*s[7,4,1^6] + 12324*s[7,3^3,1] + 15024*s[7,3^2,2^2] + 27929*s[7,3^2,2,1^2] + 14633*s[7,3^2,1^4] + 18826*s[7,3,2^3,1] + 21568*s[7,3,2^2,1^3] + 11767*s[7,3,2,1^5] + 3010*s[7,3,1^7] + 3085*s[7,2^5] + 6592*s[7,2^4,1^2] + 5919*s[7,2^3,1^4] + 2964*s[7,2^2,1^6] + 886*s[7,2,1^8] + 100*s[7,1^10] + 996*s[6^2,5] + 6055*s[6^2,4,1] + 9532*s[6^2,3,2] + 12138*s[6^2,3,1^2] + 11558*s[6^2,2^2,1] + 10172*s[6^2,2,1^3] + 3103*s[6^2,1^5] + 4323*s[6,5^2,1] + 15183*s[6,5,4,2] + 18350*s[6,5,4,1^2] + 10860*s[6,5,3^2] + 40260*s[6,5,3,2,1] + 28256*s[6,5,3,1^3] + 15426*s[6,5,2^3] + 29744*s[6,5,2^2,1^2] + 19093*s[6,5,2,1^4] + 4831*s[6,5,1^6] + 9126*s[6,4^2,3] + 27641*s[6,4^2,2,1] + 18166*s[6,4^2,1^3] + 26614*s[6,4,3^2,1] + 30913*s[6,4,3,2^2] + 55783*s[6,4,3,2,1^2] + 28479*s[6,4,3,1^4] + 29912*s[6,4,2^3,1] + 33424*s[6,4,2^2,1^3] + 17561*s[6,4,2,1^5] + 3977*s[6,4,1^7] + 12368*s[6,3^3,2] + 18249*s[6,3^3,1^2] + 28507*s[6,3^2,2^2,1] + 29932*s[6,3^2,2,1^3] + 12649*s[6,3^2,1^5] + 10354*s[6,3,2^4] + 22440*s[6,3,2^3,1^2] + 19005*s[6,3,2^2,1^4] + 8835*s[6,3,2,1^6] + 1986*s[6,3,1^8] + 4863*s[6,2^5,1] + 6363*s[6,2^4,1^3] + 4630*s[6,2^3,1^5] + 2081*s[6,2^2,1^7] + 569*s[6,2,1^9] + 70*s[6,1^11] + 3196*s[5^3,2] + 3910*s[5^3,1^2] + 6517*s[5^2,4,3] + 19140*s[5^2,4,2,1] + 12430*s[5^2,4,1^3] + 15487*s[5^2,3^2,1] + 17222*s[5^2,3,2^2] + 31211*s[5^2,3,2,1^2] + 15460*s[5^2,3,1^4] + 15658*s[5^2,2^3,1] + 17496*s[5^2,2^2,1^3] + 8958*s[5^2,2,1^5] + 2052*s[5^2,1^7] + 2312*s[5,4^3] + 16404*s[5,4^2,3,1] + 15555*s[5,4^2,2^2] + 27001*s[5,4^2,2,1^2] + 12745*s[5,4^2,1^4] + 19295*s[5,4,3^2,2] + 28120*s[5,4,3^2,1^2] + 41140*s[5,4,3,2^2,1] + 42412*s[5,4,3,2,1^3] + 17242*s[5,4,3,1^5] + 11914*s[5,4,2^4] + 25422*s[5,4,2^3,1^2] + 21182*s[5,4,2^2,1^4] + 9412*s[5,4,2,1^6] + 1952*s[5,4,1^8] + 3971*s[5,3^4] + 18844*s[5,3^3,2,1] + 15423*s[5,3^3,1^3] + 12560*s[5,3^2,2^3] + 26701*s[5,3^2,2^2,1^2] + 20544*s[5,3^2,2,1^4] + 7499*s[5,3^2,1^6] + 12818*s[5,3,2^4,1] + 16526*s[5,3,2^3,1^3] + 11397*s[5,3,2^2,1^5] + 4716*s[5,3,2,1^7] + 938*s[5,3,1^9] + 1839*s[5,2^6] + 4128*s[5,2^5,1^2] + 4190*s[5,2^4,1^4] + 2580*s[5,2^3,1^6] + 1097*s[5,2^2,1^8] + 268*s[5,2,1^10] + 44*s[5,1^12] + 2339*s[4^4,1] + 6632*s[4^3,3,2] + 9369*s[4^3,3,1^2] + 11200*s[4^3,2^2,1] + 11122*s[4^3,2,1^3] + 4177*s[4^3,1^5] + 3263*s[4^2,3^3] + 15704*s[4^2,3^2,2,1] + 12880*s[4^2,3^2,1^3] + 9934*s[4^2,3,2^3] + 20531*s[4^2,3,2^2,1^2] + 15720*s[4^2,3,2,1^4] + 5383*s[4^2,3,1^6] + 8121*s[4^2,2^4,1] + 10292*s[4^2,2^3,1^3] + 7091*s[4^2,2^2,1^5] + 2788*s[4^2,2,1^7] + 570*s[4^2,1^9] + 4504*s[4,3^4,1] + 6342*s[4,3^3,2^2] + 12385*s[4,3^3,2,1^2] + 7485*s[4,3^3,1^4] + 10901*s[4,3^2,2^3,1] + 13518*s[4,3^2,2^2,1^3] + 8560*s[4,3^2,2,1^5] + 2734*s[4,3^2,1^7] + 3273*s[4,3,2^5] + 7562*s[4,3,2^4,1^2] + 7371*s[4,3,2^3,1^4] + 4431*s[4,3,2^2,1^6] + 1669*s[4,3,2,1^8] + 331*s[4,3,1^10] + 1529*s[4,2^6,1] + 2142*s[4,2^5,1^3] + 1791*s[4,2^4,1^5] + 987*s[4,2^3,1^7] + 388*s[4,2^2,1^9] + 89*s[4,2,1^11] + 11*s[4,1^13] + 1055*s[3^5,2] + 1546*s[3^5,1^2] + 2925*s[3^4,2^2,1] + 3307*s[3^4,2,1^3] + 1702*s[3^4,1^5] + 1414*s[3^3,2^4] + 3353*s[3^3,2^3,1^2] + 3069*s[3^3,2^2,1^4] + 1732*s[3^3,2,1^6] + 468*s[3^3,1^8] + 1440*s[3^2,2^5,1] + 2049*s[3^2,2^4,1^3] + 1642*s[3^2,2^3,1^5] + 926*s[3^2,2^2,1^7] + 318*s[3^2,2,1^9] + 81*s[3^2,1^11] + 259*s[3,2^7] + 575*s[3,2^6,1^2] + 654*s[3,2^5,1^4] + 456*s[3,2^4,1^6] + 249*s[3,2^3,1^8] + 82*s[3,2^2,1^10] + 25*s[3,2,1^12] + 67*s[2^8,1] + 94*s[2^7,1^3] + 95*s[2^6,1^5] + 57*s[2^5,1^7] + 37*s[2^4,1^9] + 11*s[2^3,1^11] + 7*s[2^2,1^13] + 2*s[1^17]

==> Tables_of_results.tex <==
\section{Presentation of data}\label{sec:all-tables}
\begin{table}[htb]
    \begin{tabular}{|c|l|}
\hline
$\SymGroup[2]$-irrep & $\GL$-equivariant multiplicities in $\gr H^1_c(F(X,2))$\\
\hline
$(2)$ & 0 \\
\hline
$(1^2)$ & $\Schur{(1)}$ \\
\hline
    \end{tabular}
    \caption{Multiplicity of each isotypic component in $\gr H_c^{1}(F(X,2))$}
    \label{table:final_answer2}
\end{table}

\begin{table}[htb]
    \begin{tabular}{|c|l|}
\hline
$\SymGroup[3]$-irrep & $\GL$-equivariant multiplicities in $\gr H^2_c(F(X,3))$\\
\hline
$(3)$ & $\Schur{(1)}$ \\
\hline
$(2,1)$ & 0 \\
\hline
$(1^3)$ & $\Schur{(2)}$ \\
\hline
    \end{tabular}
    \caption{Multiplicity of each isotypic component in $\gr H_c^{2}(F(X,3))$}
    \label{table:final_answer3}
\end{table}

\begin{table}[htb]
    \begin{tabular}{|c|l|}
\hline
$\SymGroup[4]$-irrep & $\GL$-equivariant multiplicities in $\gr H^3_c(F(X,4))$\\
\hline
$(4)$ & $\Schur{(1^2)}$ \\
\hline
$(3,1)$ & $\Schur{(2)}$ \\
\hline
$(2^2)$ & $\Schur{(1)}$ \\
\hline
$(2,1^2)$ & 0 \\
\hline
$(1^4)$ & $\Schur{(3)}$ \\
\hline
    \end{tabular}
    \caption{Multiplicity of each isotypic component in $\gr H_c^{3}(F(X,4))$}
    \label{table:final_answer4}
\end{table}

\begin{table}[htb]
    \begin{tabular}{|c|l|}
\hline
$\SymGroup[5]$-irrep & $\GL$-equivariant multiplicities in $\gr H^4_c(F(X,5))$\\
\hline
$(5)$ & $\Schur{(2)} + \Schur{(1^3)}$ \\
\hline
$(4,1)$ & 0 \\
\hline
$(3,2)$ & $\Schur{(2)} + \Schur{(1^2)}$ \\
\hline
$(3,1^2)$ & $\Schur{(3)} + \Schur{(1)}$ \\
\hline
$(2^2,1)$ & $\Schur{(2)}$ \\
\hline
$(2,1^3)$ & 0 \\
\hline
$(1^5)$ & $\Schur{(4)}$ \\
\hline
    \end{tabular}
    \caption{Multiplicity of each isotypic component in $\gr H_c^{4}(F(X,5))$}
    \label{table:final_answer5}
\end{table}

\begin{table}[htb]
    \begin{tabular}{|c|l|}
\hline
$\SymGroup[6]$-irrep & $\GL$-equivariant multiplicities in $\gr H^5_c(F(X,6))$\\
\hline
$(6)$ & $\Schur{(2,1)} + \Schur{(1^4)}$ \\
\hline
$(5,1)$ & $\Schur{(3)}$ \\
\hline
$(4,2)$ & $\Schur{(2)} + \Schur{(1^3)}$ \\
\hline
$(4,1^2)$ & $\Schur{(2)} + \Schur{(1^2)} + \Schur{(1)}$ \\
\hline
$(3^2)$ & $\Schur{(3)} + \Schur{(2,1)} + \Schur{(1)}$ \\
\hline
$(3,2,1)$ & $\Schur{(3)} + \Schur{(2)} + \Schur{(1^2)}$ \\
\hline
$(3,1^3)$ & $\Schur{(4)} + \Schur{(2)}$ \\
\hline
$(2^3)$ & $\Schur{(2)}$ \\
\hline
$(2^2,1^2)$ & $\Schur{(3)} + \Schur{(1)}$ \\
\hline
$(2,1^4)$ & 0 \\
\hline
$(1^6)$ & $\Schur{(5)}$ \\
\hline
    \end{tabular}
    \caption{Multiplicity of each isotypic component in $\gr H_c^{5}(F(X,6))$}
    \label{table:final_answer6}
\end{table}

\begin{table}[htb]
    \begin{tabular}{|c|l|}
\hline
$\SymGroup[7]$-irrep & $\GL$-equivariant multiplicities in $\gr H^6_c(F(X,7))$\\
\hline
$(7)$ & $\Schur{(3)} + \Schur{(2,1^2)} + \Schur{(1^5)}$ \\
\hline
$(6,1)$ & 0 \\
\hline
$(5,2)$ & $\Schur{(3)} + \Schur{(2,1)} + \Schur{(1^4)} + \Schur{(1)}$ \\
\hline
$(5,1^2)$ & $\Schur{(4)} + 2\Schur{(2)} + \Schur{(1^3)} + \Schur{(1^2)}$ \\
\hline
$(4,3)$ & $\Schur{(3)} + \Schur{(2)} + \Schur{(1^2)}$ \\
\hline
$(4,2,1)$ & $2\Schur{(3)} + \Schur{(2,1)} + 2\Schur{(2)} + \Schur{(1^3)} + \Schur{(1^2)} + \Schur{(1)}$ \\
\hline
$(4,1^3)$ & $\Schur{(3)} + \Schur{(2)} + \Schur{(1^2)}$ \\
\hline
$(3^2,1)$ & $\Schur{(4)} + 2\Schur{(2)} + \Schur{(1^3)} + \Schur{(1^2)}$ \\
\hline
$(3,2^2)$ & $2\Schur{(3)} + \Schur{(2,1)} + \Schur{(1)}$ \\
\hline
$(3,2,1^2)$ & $\Schur{(4)} + \Schur{(3)} + 2\Schur{(2)} + \Schur{(1^2)} + \Schur{(1)}$ \\
\hline
$(3,1^4)$ & $\Schur{(5)} + \Schur{(3)} + \Schur{(1)}$ \\
\hline
$(2^3,1)$ & $\Schur{(3)} + \Schur{(2)} + \Schur{(1^2)}$ \\
\hline
$(2^2,1^3)$ & $\Schur{(4)} + \Schur{(2)}$ \\
\hline
$(2,1^5)$ & 0 \\
\hline
$(1^7)$ & $\Schur{(6)}$ \\
\hline
    \end{tabular}
    \caption{Multiplicity of each isotypic component in $\gr H_c^{6}(F(X,7))$}
    \label{table:final_answer7}
\end{table}

\begin{table}[htb]
    \begin{tabular}{|c|l|}
\hline
$\SymGroup[8]$-irrep & $\GL$-equivariant multiplicities in $\gr H^7_c(F(X,8))$\\
\hline
$(8)$ & $\Schur{(3,1)} + \Schur{(2,1^3)} + \Schur{(1^6)}$ \\
\hline
$(7,1)$ & $\Schur{(4)}$ \\
\hline
$(6,2)$ & $\Schur{(3)} + \Schur{(2,1^2)} + \Schur{(2)} + \Schur{(1^5)} + \Schur{(1^2)} + \Schur{(1)}$ \\
\hline
$(6,1^2)$ & $\Schur{(3)} + \Schur{(2,1)} + \Schur{(2)} + \Schur{(1^4)} + \Schur{(1^3)}$ \\
\hline
$(5,3)$ & $\Schur{(4)} + 2\Schur{(2)} + \Schur{(1^3)} + \Schur{(1^2)}$ \\
\hline
$(5,2,1)$ & $\Schur{(4)} + 3\Schur{(3)} + 2\Schur{(2,1)} + 3\Schur{(2)} + \Schur{(1^4)} + \Schur{(1^3)} + 2\Schur{(1^2)} + \Schur{(1)}$ \\
\hline
$(5,1^3)$ & $\Schur{(5)} + 2\Schur{(3)} + \Schur{(2,1)} + \Schur{(2)} + \Schur{(1^3)} + \Schur{(1^2)} + \Schur{(1)}$ \\
\hline
$(4^2)$ & $2\Schur{(3)} + \Schur{(2,1)} + \Schur{(1)}$ \\
\hline
$(4,3,1)$ & $\Schur{(4)} + 3\Schur{(3)} + 2\Schur{(2,1)} + 3\Schur{(2)} + \Schur{(1^4)} + 2\Schur{(1^3)} + 2\Schur{(1^2)} + \Schur{(1)}$ \\
\hline
$(4,2^2)$ & $\Schur{(4)} + 3\Schur{(3)} + \Schur{(2,1)} + 2\Schur{(2)} + 2\Schur{(1^2)} + 2\Schur{(1)}$ \\
\hline
$(4,2,1^2)$ & $2\Schur{(4)} + 3\Schur{(3)} + \Schur{(2,1)} + 5\Schur{(2)} + 2\Schur{(1^3)} + 2\Schur{(1^2)} + \Schur{(1)}$ \\
\hline
$(4,1^4)$ & $\Schur{(4)} + \Schur{(3)} + \Schur{(2)} + \Schur{(1^2)} + \Schur{(1)}$ \\
\hline
$(3^2,2)$ & $\Schur{(4)} + \Schur{(3)} + 3\Schur{(2)} + \Schur{(1^3)} + \Schur{(1^2)}$ \\
\hline
$(3^2,1^2)$ & $\Schur{(5)} + 4\Schur{(3)} + 2\Schur{(2,1)} + \Schur{(2)} + \Schur{(1^2)} + 2\Schur{(1)}$ \\
\hline
$(3,2^2,1)$ & $2\Schur{(4)} + 2\Schur{(3)} + \Schur{(2,1)} + 3\Schur{(2)} + \Schur{(1^3)} + 2\Schur{(1^2)} + \Schur{(1)}$ \\
\hline
$(3,2,1^3)$ & $\Schur{(5)} + \Schur{(4)} + 2\Schur{(3)} + 3\Schur{(2)} + 2\Schur{(1^2)} + \Schur{(1)}$ \\
\hline
$(3,1^5)$ & $\Schur{(6)} + \Schur{(4)} + \Schur{(2)}$ \\
\hline
$(2^4)$ & $2\Schur{(3)} + \Schur{(2,1)} + \Schur{(1)}$ \\
\hline
$(2^3,1^2)$ & $\Schur{(4)} + \Schur{(3)} + \Schur{(2)}$ \\
\hline
$(2^2,1^4)$ & $\Schur{(5)} + \Schur{(3)} + \Schur{(1)}$ \\
\hline
$(2,1^6)$ & 0 \\
\hline
$(1^8)$ & $\Schur{(7)}$ \\
\hline
    \end{tabular}
    \caption{Multiplicity of each isotypic component in $\gr H_c^{7}(F(X,8))$}
    \label{table:final_answer8}
\end{table}

\begin{table}[htb]
    \begin{tabular}{|m{1.5cm}|m{11cm}|}
\hline
$\SymGroup[9]$-irrep & $\GL$-equivariant multiplicities in $\gr H^8_c(F(X,9))$\\
\hline
$(9)$ & $\Schur{(4)} + \Schur{(3,1^2)} + \Schur{(2,1^4)} + \Schur{(1^7)}$ \\
\hline
$(8,1)$ & 0 \\
\hline
$(7,2)$ & $\Schur{(4)} + \Schur{(3,1)} + \Schur{(2,1^3)} + 2\Schur{(2)} + \Schur{(1^6)} + \Schur{(1^3)} + \Schur{(1^2)}$ \\
\hline
$(7,1^2)$ & $\Schur{(5)} + 2\Schur{(3)} + \Schur{(2,1^2)} + \Schur{(2,1)} + \Schur{(1^5)} + \Schur{(1^4)} + \Schur{(1)}$ \\
\hline
$(6,3)$ & $\Schur{(4)} + 2\Schur{(3)} + 2\Schur{(2,1)} + 2\Schur{(2)} + \Schur{(1^4)} + \Schur{(1^3)} + \Schur{(1^2)} + \Schur{(1)}$ \\
\hline
$(6,2,1)$ & $2\Schur{(4)} + 4\Schur{(3)} + \Schur{(2,1^2)} + 2\Schur{(2,1)} + 4\Schur{(2)} + \Schur{(1^5)} + \Schur{(1^4)} + 2\Schur{(1^3)} + 3\Schur{(1^2)} + \Schur{(1)}$ \\
\hline
$(6,1^3)$ & $\Schur{(4)} + 2\Schur{(3)} + 2\Schur{(2,1)} + 2\Schur{(2)} + \Schur{(1^4)} + \Schur{(1^3)} + \Schur{(1^2)} + \Schur{(1)}$ \\
\hline
$(5,4)$ & $\Schur{(4)} + \Schur{(3)} + 2\Schur{(2)} + \Schur{(1^3)} + 2\Schur{(1^2)}$ \\
\hline
$(5,3,1)$ & $\Schur{(5)} + \Schur{(4)} + 8\Schur{(3)} + \Schur{(2,1^2)} + 5\Schur{(2,1)} + 5\Schur{(2)} + \Schur{(1^5)} + 2\Schur{(1^4)} + 3\Schur{(1^3)} + 3\Schur{(1^2)} + 3\Schur{(1)}$ \\
\hline
$(5,2^2)$ & $4\Schur{(4)} + \Schur{(3,1)} + 2\Schur{(3)} + \Schur{(2,1)} + 7\Schur{(2)} + 3\Schur{(1^3)} + 4\Schur{(1^2)} + \Schur{(1)}$ \\
\hline
$(5,2,1^2)$ & $\Schur{(5)} + 3\Schur{(4)} + 8\Schur{(3)} + 5\Schur{(2,1)} + 6\Schur{(2)} + 2\Schur{(1^4)} + 3\Schur{(1^3)} + 4\Schur{(1^2)} + 3\Schur{(1)}$ \\
\hline
$(5,1^4)$ & $\Schur{(6)} + 2\Schur{(4)} + \Schur{(3)} + 4\Schur{(2)} + 2\Schur{(1^3)} + 2\Schur{(1^2)}$ \\
\hline
$(4^2,1)$ & $3\Schur{(4)} + \Schur{(3,1)} + 2\Schur{(3)} + 2\Schur{(2,1)} + 4\Schur{(2)} + \Schur{(1^4)} + 2\Schur{(1^3)} + 2\Schur{(1^2)} + \Schur{(1)}$ \\
\hline
$(4,3,2)$ & $3\Schur{(4)} + 7\Schur{(3)} + 4\Schur{(2,1)} + 6\Schur{(2)} + \Schur{(1^4)} + 3\Schur{(1^3)} + 4\Schur{(1^2)} + 2\Schur{(1)}$ \\
\hline
$(4,3,1^2)$ & $\Schur{(5)} + 4\Schur{(4)} + 8\Schur{(3)} + 4\Schur{(2,1)} + 8\Schur{(2)} + \Schur{(1^4)} + 3\Schur{(1^3)} + 5\Schur{(1^2)} + 3\Schur{(1)}$ \\
\hline
$(4,2^2,1)$ & $\Schur{(5)} + 4\Schur{(4)} + 8\Schur{(3)} + 4\Schur{(2,1)} + 8\Schur{(2)} + \Schur{(1^4)} + 3\Schur{(1^3)} + 5\Schur{(1^2)} + 3\Schur{(1)}$ \\
\hline
$(4,2,1^3)$ & $2\Schur{(5)} + 3\Schur{(4)} + 7\Schur{(3)} + 3\Schur{(2,1)} + 6\Schur{(2)} + 2\Schur{(1^3)} + 4\Schur{(1^2)} + 3\Schur{(1)}$ \\
\hline
$(4,1^5)$ & $\Schur{(5)} + \Schur{(4)} + \Schur{(3)} + 2\Schur{(2)} + \Schur{(1^2)} + \Schur{(1)}$ \\
\hline
$(3^3)$ & $\Schur{(5)} + 3\Schur{(3)} + 3\Schur{(2,1)} + \Schur{(1^4)} + 2\Schur{(1)}$ \\
\hline
$(3^2,2,1)$ & $\Schur{(5)} + 3\Schur{(4)} + 6\Schur{(3)} + 2\Schur{(2,1)} + 6\Schur{(2)} + 2\Schur{(1^3)} + 4\Schur{(1^2)} + 2\Schur{(1)}$ \\
\hline
$(3^2,1^3)$ & $\Schur{(6)} + 4\Schur{(4)} + 2\Schur{(3)} + \Schur{(2,1)} + 6\Schur{(2)} + 2\Schur{(1^3)} + 3\Schur{(1^2)} + \Schur{(1)}$ \\
\hline
$(3,2^3)$ & $3\Schur{(4)} + \Schur{(3,1)} + 2\Schur{(3)} + \Schur{(2,1)} + 4\Schur{(2)} + \Schur{(1^3)} + 2\Schur{(1^2)} + \Schur{(1)}$ \\
\hline
$(3,2^2,1^2)$ & $2\Schur{(5)} + 2\Schur{(4)} + 7\Schur{(3)} + 3\Schur{(2,1)} + 4\Schur{(2)} + \Schur{(1^3)} + 2\Schur{(1^2)} + 3\Schur{(1)}$ \\
\hline
$(3,2,1^4)$ & $\Schur{(6)} + \Schur{(5)} + 2\Schur{(4)} + 3\Schur{(3)} + 3\Schur{(2)} + 2\Schur{(1^2)} + \Schur{(1)}$ \\
\hline
$(3,1^6)$ & $\Schur{(7)} + \Schur{(5)} + \Schur{(3)} + \Schur{(1)}$ \\
\hline
$(2^4,1)$ & $2\Schur{(4)} + \Schur{(3)} + \Schur{(2)} + \Schur{(1^2)}$ \\
\hline
$(2^3,1^3)$ & $\Schur{(5)} + \Schur{(4)} + \Schur{(3)} + 2\Schur{(2)} + \Schur{(1^2)} + \Schur{(1)}$ \\
\hline
$(2^2,1^5)$ & $\Schur{(6)} + \Schur{(4)} + \Schur{(2)}$ \\
\hline
$(2,1^7)$ & 0 \\
\hline
$(1^9)$ & $\Schur{(8)}$ \\
\hline
    \end{tabular}
    \caption{Multiplicity of each isotypic component in $\gr H_c^{8}(F(X,9))$}
    \label{table:final_answer9}
\end{table}

